Generative Modeling with Phase Stochastic Bridges

Diffusion models (DMs) represent state-of-the-art generative models for continuous inputs. DMs work by constructing a Stochastic Differential Equation (SDE) in the input space (ie, position space), and using a neural network to reverse it. In this work, we introduce a novel generative modeling framework grounded in \textbf{phase space dynamics}, where a phase space is defined as {an augmented space encompassing both position and velocity.} Leveraging insights from Stochastic Optimal Control, we construct a path measure in the phase space that enables efficient sampling. {In contrast to DMs, our framework demonstrates the capability to generate realistic data points at an early stage of dynamics propagation.} This early prediction sets the stage for efficient data generation by leveraging additional velocity information along the trajectory. On standard image generation benchmarks, our model yields favorable performance over baselines in the regime of small Number of Function Evaluations (NFEs). Furthermore, our approach rivals the performance of diffusion models equipped with efficient sampling techniques, underscoring its potential as a new tool generative modeling.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> subtex/abstract.tex <==
Diffusion models (DMs) represent state-of-the-art generative models for continuous inputs. DMs work by constructing a Stochastic Differential Equation (SDE) in the input space (ie, position space), and using a neural network to reverse it. In this work, we introduce a novel generative modeling framework grounded in \textbf{phase space dynamics}, where a phase space is defined as {an augmented space encompassing both position and velocity.} Leveraging insights from Stochastic Optimal Control, we construct a path measure in the phase space that enables efficient sampling. {In contrast to DMs, our framework demonstrates the capability to generate realistic data points at an early stage of dynamics propagation.} This early prediction sets the stage for efficient data generation by leveraging additional velocity information along the trajectory. On standard image generation benchmarks, our model yields favorable performance over baselines in the regime of small Number of Function Evaluations (NFEs). Furthermore, our approach rivals the performance of diffusion models equipped with efficient sampling techniques, underscoring its potential as a new tool generative modeling.   

==> subtex/results_imagenet.tex <==
\section{Experimental Results}\label{Sec:exp}
\textbf{Architectures and Hyperparameters} We parameterize $\rvs_t^{\theta}(\cdot,\cdot;\theta)$ using modified NCSN++ model as provided in \cite{karras2022elucidating}. We employ six input channels, accounting for both position and velocity variables, as opposed to the standard three channels used in the CIFAR-10 \citep{krizhevsky2009learning}, AFHQv2 \citep{choi2020stargan} and ImageNet\citep{deng2009imagenet} which leads to a negligible increase of network parameters. For the purpose of comparison with CLD in the toy dataset, we adopt the same ResNet-based architecture utilized in CLD. Throughout all of our experiments, we maintain a monotonically decreasing diffusion coefficient, given by $g(t) = 3(1-t)$. For the detailed experimental setup, please refer to Appendix.\ref{Appendix:exp}.

\textbf{Evaluation}: To assess the performance and the sampling speed of various algorithms, we employ the Fréchet Inception Distance score (FID;\cite{heusel2017gans}) and the Number of Function Evaluations (NFE) as our metrics. For FID evaluation, we utilize reference statistics for CIFAR-10 and AFHQv2 obtained from the EDM \citep{karras2022elucidating} and compare our results with it using 50,000 generated samples. Additionally, we re-evaluate the FID of CLD using the same reference statistics to ensure consistency in our comparisons. For all other reported values, we directly source them from the respective referenced papers.


%  We empirically validate the efficacy of our proposed model in the context of generative modeling tasks. Through experimentation with intricate toy datasets, we demonstrate its superior performance compared to the baseline CLD, even when utilizing significantly fewer Number of Function Evaluations (NFEs) by using same stochastic sampler. Such benefits is also kept for high dimensional CIFAR-10 dataset. Additionally, we conduct experiments with deterministic sampling techniques on the CIFAR10 and AFHQv2 datasets, yielding compelling results that stand out in comparison to prior works which are specially designed for the fast sampling of diffusion model.
% \begin{figure}[t]
%     \includegraphics[width=\textwidth]{figs/cld_am_toy.pdf}
%     \caption{The comparison with CLD\citep{dockhorn2021score} using same network and stochastic sampler SSS, for Multi-Swiss-Roll and Mixture of Gaussian datasets. We achieve visually better results with one order less NFEs.}
%     \label{fig:cld-am-toy}
%     \vskip -0.05in
% \end{figure}
\begin{figure}[t]
    \hspace*{1.3cm}
    \includegraphics[width=0.8\textwidth]{figs/random_smaple_cifar10_afhqv2.pdf}
    \caption{Uncurated sample from CIFAR-10 (left) and AFHQv2 (right) generated from AGM-ODE.}
    \label{fig:random-samples}
\end{figure}

\begin{figure}[t]
    \includegraphics[width=\textwidth]{figs/EDM_AM_NFE_comparison.pdf}
    \caption{Comparison with EDM \citep{karras2022elucidating} on AFHQv2 dataset. AGM-ODE exhibits superior generative performance when NFE is exceedingly low, owing to its unique dynamics architecture that incorporates velocity when predicting the estimated data point. We have normalized the output of EDM when NFE is 5 to facilitate clearer visualization.}
    \label{fig:NFE_ablation}
\end{figure}

% \begin{figure}[t]
%     \includegraphics[width=\textwidth]{figs/EDM_AM_NFE_comparison.pdf}
%     \caption{Random sample from AFHQv2 and cifar10}
%     \label{fig:random-samples}
% \end{figure}
% \begin{wraptable}{r}{0.3\textwidth} % {position}{width}
%     \centering
%     \begin{tabular}{ccccc}
%         \toprule
%         NFE &  50 & 100& 150  \\[1pt]
%         \hline
%         CLD  & XX & XXX&XX \\[1pt]
%         AGM  & XX&XX&XX \\[1pt]
%         % CLD \cite{dockhorn2021score} & \xmark & $p_\calA(x) \otimes \mathcal{N}(\mathbf{0},\bm{\Sigma}) $ &  $\mathcal{N}(\mathbf{0},\bm{\Sigma}) \otimes \mathcal{N}(\mathbf{0},\bm{\Sigma})$ \\[1pt]
%         % % \bottomrule
%         % SB \cite{chen2021likelihood} & $\downarrow W_2\rightarrow$ kinks & $p_\calA(x)$ & $p_\calB(x)$ \\[1pt]
%         % DMSB (ours)  & $\downarrow W_2\rightarrow$ smooth& $p_\calA(x) q_\theta(v|x) $ & $p_\calB(x) q_\phi(v|x)$\\[1pt]
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison with CLD using same stochastic sampler SSCS in Cifar10 generative task.}
%   \end{wraptable}
% \begin{table}[t]
%     \caption{Comparision with CLD with same Stochastic Symmetric Splitting Sampler.
%     }\label{table:sscs-sampler}
%     \begin{center}
%         \begin{tabular}{ccccc}
%             \toprule
%             NFE &  20 &50 & 150  &1000\\[1pt]
%             \hline
%             CLD \citep{dockhorn2021score}   &N/A& 20.5 & 3.07 & 2.23 \\[1pt]
%             AGM(ours)                       &7.9 & 3.21 & 2.68 & 2.46 \\[1pt]
%             \bottomrule
%         \end{tabular}
%     \end{center}
% \end{table}
\begin{wraptable}{r}{0.4\textwidth}
\caption{FID$\downarrow$ Comparison with CLD\citep{dockhorn2021score} using same SSS Sampler on CIFAR-10.}\label{table:sscs-sampler}
\begin{tabular}{ccc}\\\toprule  
NFE$\downarrow$ & CLD-SDE & AGM-SDE \\\midrule
20      &$>$100 & 7.9\\  \midrule
50      &19.93 & 3.21\\  \midrule
150     &2.99 & 2.68\\  \midrule
1000    &2.44 & 2.46\\  \bottomrule
\end{tabular}
\end{wraptable} 
\begin{table}[t]
    \caption{Performance comparing with other algorithm using FID$\downarrow$ metric on CIFAR-10}\label{table:small-NFE}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|}
    \toprule
                & &NFE$\downarrow$&5 & 10 & 20\\
    \hline
    Dynamics Order & Model Name\\
    \hline
    \multirow{4}{*}{\begin{tabular}{c}1st order\\dynamics\end{tabular}} & EDM \citep{karras2022elucidating} &&$>$ 100 &15.78 & \textbf{2.23} \\
                                                                        & VP+EI \citep{zhang2022fast} &&15.37 &\textbf{4.17} &3.03 \\
                                                                        & DDIM \citep{song2020denoising} &&26.91 &11.14&3.50 \\
                                                                        &Analytic-DPM\citep{bao2022analytic}&&51.47 &14.06 &6.74\\
                                                                        &RES\citep{zhang2023improved}&&14.32 &5.12 &2.54\\
    \hline
    \hline
    \multirow{2}{*}{\begin{tabular}{c}2nd order\\dynamics\end{tabular}} & CLD+EI \citep{zhang2022gddim} &&N/A &13.41 & 3.39 \\
                                                                        & \textbf{AGM-ODE(ours)}            &&\textbf{11.93} &4.60 &2.60 \\
    \bottomrule
\end{tabular}
\end{table}
\textbf{Stochastic Sampling:} In our experiments, we emphasize the advantages of employing the AGM-SDE in comparison to CLD. Firstly, we establish that our model exhibits superior performance when the Number of Function Evaluations (NFE) is significantly lower than that of CLD, particularly in toy dataset scenarios. For evaluation, we utilized the multi-modal Mixture of Gaussian and Multi-Swiss-Roll datasets. The results obtained from the toy dataset, as shown in Fig.\ref{fig:cld-am-toy}, demonstrate that AGM is capable of generating data that closely aligns with the ground truth, while requiring NFE that is around one order of magnitude lower than CLD. Furthermore, our findings reveal that AGM outperforms CLD in the context of CIFAR-10 image generation tasks, especially when faced with limited NFE, as illustrated in Table \ref{table:sscs-sampler}.

\textbf{Deterministic Sampling:} Next, we validate our algorithm on high-dimensional image generation with a  deterministic sampler. The generated images for CIFAR-10 and AFHQv2 are presented in Fig.\ref{fig:random-samples}, which clearly suggest that AGM-ODE is able to synthesize high-fidelity images. More uncurated images can be found in Appendix.\ref{Appendix:figs}.  Regarding the quantitative evaluation, Table.\ref{table:all-results} summarizes
the FID together with NFE used for sampling on CIFAR-10.  Notably, AGM-ODE achieves 2.46 FID score on
CIFAR-10, which is comparable to the existing dynamical generative modeling and outperforms prior 2nd-order dynamics methods \citep{dockhorn2021score,zhang2022gddim}. 

We underscore the effectiveness of sampling-hop, especially when faced with a constrained NFE budget, in comparison to the standard Diffusion Model. We validate it on the CIFAR-10 and AFHQv2 dataset respectively. Fig.\ref{fig:NFE_ablation} illustrates that AGM-ODE is able to generate plausible images even when NFE$=5$ and outperforms EDM\citep{karras2022elucidating} when NFE is extremely small (NFE$<$15) visually and numerically on AFHQv2 dataset. We also compare with other fast sampling algorithms built upon DM in table.\ref{table:small-NFE} on CIFAR-10 dataset where AGM-ODE demonstrates competitive performance. Notably, AGM-ODE outperforms the baseline CLD with the same EI sampler by a large margin. We suspect that the improvement is based on the rectified trajectory which is more friendly for the ODE solver.

% \begin{wraptable}{r}{0.4\textwidth}
%     \caption{Unconditional ImageNet64 generative performance using FID$\downarrow$ metric}\label{Imagenet}
%     \begin{tabular}{lll}\\\toprule  
%     Model& NFE$\downarrow$ & FID$\downarrow$ \\\midrule
%     DDPM\citep{ho2020denoising}        &264 & 17.36\\  \midrule
%     ScoreFlow\citep{song2021maximum}   &601 & 24.95\\  \midrule
%     FM-OT\citep{lipman2022flow}       &138 & 14.45\\  \midrule
%     FM-multismaple\citep{pooladian2023multisample}   &132 & 11.82\\  \midrule
%     AGM-ODE     &TBD & TBD\\  \bottomrule
%     \end{tabular}
%     \end{wraptable} 
Table \ref{table:all-results} presents a performance comparison for unconditional CIFAR-10 generative tasks when the NFE is sufficiently large. In this scenario, AGM achieves results that are comparable to those of other existing diffusion models.

% \begin{table}[htbp]
%     \caption{ODE sampler
%     }\label{table:ode-sampler}
%     \begin{center}
%         \begin{tabular}{ccccc}
%             \toprule
%             NFE &  5 & 10 & 20  \\[1pt]
%             \hline
%             EDM \citep{karras2022elucidating}  & $>100$ & 15.779 &2.23 \\[1pt]
%             VP+EI \citep{zhang2022fast}  & 15.37 & 4.17&3.03 \\[1pt]
%             CLD+EI \citep{zhang2022gddim}  & N/A & 13.41&3.39 \\[1pt]
%             AGM(ours) +EI  & 16.25 & 6.25&XXX \\[1pt]
%             \bottomrule
%         \end{tabular}
%     \end{center}
% \end{table}

\begin{table}[t]
    \centering
    \caption{Unconditional ImageNet64 generative performance using FID$\downarrow$ metric}\label{Imagenet}
    \begin{tabular}{lll}\\\toprule  
    Model& NFE$\downarrow$ & FID$\downarrow$ \\\midrule
    DDPM\citep{ho2020denoising}        &264 & 17.36\\  \midrule
    ScoreFlow\citep{song2021maximum}   &601 & 24.95\\  \midrule
    FM-OT\citep{lipman2022flow}       &138 & 14.45\\  \midrule
    FM-multismaple\citep{pooladian2023multisample}   &132 & 11.82\\  \midrule
    AGM-ODE(ours)     &TBD & TBD\\  \bottomrule
    \end{tabular}
    \end{table}
    
\begin{table}[t]
\caption{Unconditional CIFAR-10 generative performance using FID$\downarrow$ metric}\label{table:all-results}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\toprule
Dynamics Type & Model Name&NFE$\downarrow$&FID$\downarrow$\\
\hline
\multirow{4}{*}{\begin{tabular}{c}ODE\end{tabular}}                 & EDM \citep{karras2022elucidating} & 35 &1.84\\
                                                                    & CLD+ODE \citep{zhang2022gddim} & 312&2.25  \\
                                                                    & Flow Matching \citep{zhang2022gddim} &142 &6.35  \\
                                                                    & VP-GGF \citep{jolicoeur2021gotta} &330 &2.56  \\
                                                                    & VE-GGF \citep{jolicoeur2021gotta} &488 &2.99  \\
                                                                    & \textbf{AGM-ODE(ours)}            &50& 2.46\\
\hline
\hline
\multirow{2}{*}{\begin{tabular}{c}SDE\end{tabular}}                 & DDPM \citep{ho2020denoising}  &1000&3.17\\
                                                                    & CLD \citep{dockhorn2021score}             &1000& 2.44\\
                                                                    & \textbf{AGM-SDE(ours)}            &1000& 2.46\\
\bottomrule
\end{tabular}
\end{table}



    
